Challenges and Opportunities in Multi-device Speech Processing

We review current solutions and technical challenges for automatic speech recognition, keyword spotting, device arbitration, speech enhancement, and source localization in multidevice home environments to provide context for the INTERSPEECH 2022 special session, "Challenges and opportunities for signal processing and machine learning for multiple smart devices". We also identify the datasets needed to support these research areas. Based on the review and our research experience in the multi-device domain, we conclude with an outlook on the future evolution

==> mybib.long.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
@inproceedings{Guggenberger2015AnAO,
  title={An Analysis of Time Drift in Hand-Held Recording Devices},
  author={Mario Guggenberger and Mathias Lux and L{\'a}szl{\'o} B{\"o}sz{\"o}rm{\'e}nyi},
  booktitle={MMM},
  year={2015}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
@inproceedings{Yoshioka2019MeetingTU,
  title={Meeting Transcription Using Asynchronous Distant Microphones},
  author={Takuya Yoshioka and Dimitrios Dimitriadis and Andreas Stolcke and William Hinthorn and Zhuo Chen and Michael Zeng and Xuedong Huang},
  booktitle={INTERSPEECH},
  year={2019}
}

@article{Weninger2021DualEncoderAW,
  title={Dual-Encoder Architecture with Encoder Selection for Joint Close-Talk and Far-Talk Speech Recognition},
  author={Felix Weninger and Marco Gaudesi and Ralf Leibold and Roberto Gemello and Puming Zhan},
  journal={2021 IEEE Automatic Speech Recognition and Understanding Workshop (ASRU)},
  year={2021},
  pages={534-540}
}

@inproceedings{BentezGuijarro2019CoordinationOS,
  title={Coordination of Speech Recognition Devices in Intelligent Environments with Multiple Responsive Devices},
  author={Antonio Ben{\'i}tez-Guijarro and Zoraida Callejas Carri{\'o}n and Manuel Noguera and Kawtar Benghazi Akhlaki},
  booktitle={UCAmI},
  year={2019}
}

@INPROCEEDINGS{1997fiscus, author={Fiscus, J.G.}, 
booktitle={1997 IEEE Workshop on Automatic Speech Recognition and Understanding Proceedings}, 
title={A post-processing system to yield reduced word error rates: Recognizer Output Voting Error Reduction (ROVER)}, year={1997}, volume={}, number={}, pages={347-354}, doi={10.1109/ASRU.1997.659110}}

@inproceedings{Evermann2000PosteriorPD,
  title={Posterior probability decoding, confidence estimation and system combination},
  author={Gunnar Evermann and Philip C. Woodland},
  booktitle={Proc. Speech Transcription Workshop},
  volume={27},
  pages={78--81},
  year={2000},
  organization={Citeseer}
}

@article{Zhang2020PushingTL,
  title={Pushing the Limits of Semi-Supervised Learning for Automatic Speech Recognition},
  author={Yu Zhang and James Qin and Daniel S. Park and Wei Han and Chung-Cheng Chiu and Ruoming Pang and Quoc V. Le and Yonghui Wu},
  journal={ArXiv},
  year={2020},
  volume={abs/2010.10504}
}

@misc{wersoa,
  author = {{Papers with Code}},
  title = {Speech Recognition on LibriSpeech test-clean},
  year = 2022,
  url = {https://paperswithcode.com/sota/speech-recognition-on-librispeech-test-clean},
  note = {2022-03-04}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
@book{loizou2007speech,
  title={Speech enhancement: theory and practice},
  author={Loizou, Philipos C},
  year={2007},
  publisher={CRC press}
}

@article{gannot2017consolidated,
  title={A consolidated perspective on multimicrophone speech enhancement and source separation},
  author={Gannot, Sharon and Vincent, Emmanuel and Markovich-Golan, Shmulik and Ozerov, Alexey},
  journal={IEEE/ACM Transactions on Audio, Speech, and Language Processing},
  volume={25},
  number={4},
  pages={692--730},
  year={2017},
  publisher={IEEE}
}

@article{haeb2019speech,
  title={Speech processing for digital home assistants: Combining signal processing with deep-learning techniques},
  author={Haeb-Umbach, Reinhold and Watanabe, Shinji and Nakatani, Tomohiro and Bacchiani, Michiel and Hoffmeister, Bjorn and Seltzer, Michael L and Zen, Heiga and Souden, Mehrez},
  journal={IEEE Signal processing magazine},
  volume={36},
  number={6},
  pages={111--124},
  year={2019},
  publisher={IEEE}
}

@misc{ramakrishnan2015speech,
  title={Speech enhancement using multiple microphones on multiple devices},
  author={Ramakrishnan, Dinesh and Wang, Song},
  year={2015},
  month=aug # "~18",
  publisher={Google Patents},
  note={US Patent 9,113,240}
}

@inproceedings{araki2018comparison,
  title={Comparison of reference microphone selection algorithms for distributed microphone array based speech enhancement in meeting recognition scenarios},
  author={Araki, Shoko and Ono, Nobutaka and Kinoshita, Keisuke and Delcroix, Marc},
  booktitle={2018 16th International Workshop on Acoustic Signal Enhancement (IWAENC)},
  pages={316--320},
  year={2018},
  organization={IEEE}
}

@article{zhang2020study,
  title={A study on reference microphone selection for multi-microphone speech enhancement},
  author={Zhang, Jie and Chen, Huawei and Dai, Li-Rong and Hendriks, Richard Christian},
  journal={IEEE/ACM Transactions on Audio, Speech, and Language Processing},
  volume={29},
  pages={671--683},
  year={2020},
  publisher={IEEE}
}

@inproceedings{casebeer2021communication,
  title={Communication-cost aware microphone selection for neural speech enhancement with ad-hoc microphone arrays},
  author={Casebeer, Jonah and Kaikaus, Jamshed and Smaragdis, Paris},
  booktitle={ICASSP 2021-2021 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={8438--8442},
  year={2021},
  organization={IEEE}
}

@inproceedings{heymann2016neural,
  title={Neural network based spectral mask estimation for acoustic beamforming},
  author={Heymann, Jahn and Drude, Lukas and Haeb-Umbach, Reinhold},
  booktitle={2016 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={196--200},
  year={2016},
  organization={IEEE}
}

@inproceedings{higuchi2016robust,
  title={Robust MVDR beamforming using time-frequency masks for online/offline ASR in noise},
  author={Higuchi, Takuya and Ito, Nobutaka and Yoshioka, Takuya and Nakatani, Tomohiro},
  booktitle={2016 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={5210--5214},
  year={2016},
  organization={IEEE}
}

@inproceedings{meng2017deep,
  title={Deep long short-term memory adaptive beamforming networks for multichannel robust speech recognition},
  author={Meng, Zhong and Watanabe, Shinji and Hershey, John R and Erdogan, Hakan},
  booktitle={2017 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={271--275},
  year={2017},
  organization={IEEE}
}

@inproceedings{tolooshams2020channel,
  title={Channel-attention dense u-net for multichannel speech enhancement},
  author={Tolooshams, Bahareh and Giri, Ritwik and Song, Andrew H and Isik, Umut and Krishnaswamy, Arvindh},
  booktitle={ICASSP 2020-2020 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={836--840},
  year={2020},
  organization={IEEE}
}

@article{zhang2021microphone,
  title={Microphone array generalization for multichannel narrowband deep speech enhancement},
  author={Zhang, Siyuan and Li, Xiaofei},
  journal={arXiv preprint arXiv:2107.12601},
  year={2021}
}

@article{pandey2021tadrn,
  title={TADRN: Triple-Attentive Dual-Recurrent Network for Ad-hoc Array Multichannel Speech Enhancement},
  author={Pandey, Ashutosh and Xu, Buye and Kumar, Anurag and Donley, Jacob and Calamia, Paul and Wang, DeLiang},
  journal={arXiv preprint arXiv:2110.11844},
  year={2021}
}

@article{taherian2021one,
  title={One model to enhance them all: array geometry agnostic multi-channel personalized speech enhancement},
  author={Taherian, Hassan and Eskimez, Sefik Emre and Yoshioka, Takuya and Wang, Huaming and Chen, Zhuo and Huang, Xuedong},
  journal={arXiv preprint arXiv:2110.10330},
  year={2021}
}

@article{wang2019distributed,
  title={Distributed Microphone Speech Enhancement based on Deep Learning},
  author={Wang, Syu-Siang and Liang, Yu-You and Hung, Jeih-weih and Tsao, Yu and Wang, Hsin-Min and Fang, Shih-Hau},
  journal={arXiv preprint arXiv:1911.08153},
  year={2019}
}

@article{ali2021integrated,
  title={An integrated MVDR beamformer for speech enhancement using a local microphone array and external microphones},
  author={Ali, Randall and van Waterschoot, Toon and Moonen, Marc},
  journal={EURASIP Journal on Audio, Speech, and Music Processing},
  volume={2021},
  number={1},
  pages={1--20},
  year={2021},
  publisher={Springer}
}

@article{furnon2021dnn,
  title={DNN-based mask estimation for distributed speech enhancement in spatially unconstrained microphone arrays},
  author={Furnon, Nicolas and Serizel, Romain and Essid, Slim and Illina, Irina},
  journal={IEEE/ACM Transactions on Audio, Speech, and Language Processing},
  volume={29},
  pages={2310--2323},
  year={2021},
  publisher={IEEE}
}

@inproceedings{ayrapetian2021asynchronous,
  title={Asynchronous Acoustic Echo Cancellation Over Wireless Channels},
  author={Ayrapetian, Robert and Hilmes, Philip and Mansour, Mohamed and Kristjansson, Trausti and Murgia, Carlo},
  booktitle={ICASSP 2021-2021 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={116--120},
  year={2021},
  organization={IEEE}
}


@inproceedings{rix2001perceptual,
  title={Perceptual evaluation of speech quality (PESQ)-a new method for speech quality assessment of telephone networks and codecs},
  author={Rix, Antony W and Beerends, John G and Hollier, Michael P and Hekstra, Andries P},
  booktitle={2001 IEEE international conference on acoustics, speech, and signal processing. Proceedings (Cat. No. 01CH37221)},
  volume={2},
  pages={749--752},
  year={2001},
  organization={IEEE}
}

@inproceedings{taal2010short,
  title={A short-time objective intelligibility measure for time-frequency weighted noisy speech},
  author={Taal, Cees H and Hendriks, Richard C and Heusdens, Richard and Jensen, Jesper},
  booktitle={2010 IEEE international conference on acoustics, speech and signal processing},
  pages={4214--4217},
  year={2010},
  organization={IEEE}
}

@inproceedings{le2019sdr,
  title={SDR--half-baked or well done?},
  author={Le Roux, Jonathan and Wisdom, Scott and Erdogan, Hakan and Hershey, John R},
  booktitle={ICASSP 2019-2019 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={626--630},
  year={2019},
  organization={IEEE}
}

@article{reddy2021interspeech,
  title={Interspeech 2021 deep noise suppression challenge},
  author={Reddy, Chandan KA and Dubey, Harishchandra and Koishida, Kazuhito and Nair, Arun and Gopal, Vishak and Cutler, Ross and Braun, Sebastian and Gamper, Hannes and Aichner, Robert and Srinivasan, Sriram},
  journal={arXiv preprint arXiv:2101.01902},
  year={2021}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@ARTICLE{2019szoke, author={Szöke, Igor and Skácel, Miroslav and Mošner, 
Ladislav and Paliesek, Jakub and Černocký, Jan}, 
journal={IEEE Journal of Selected Topics in Signal Processing}, title={Building and evaluation of a real room impulse response dataset}, year={2019}, volume={13}, number={4}, pages={863-876}, 
doi={10.1109/JSTSP.2019.2917582}, note={{D}ata: \url{https://speech.fit.vutbr.cz/software/but-speech-fit-reverb-database}}}

@article{McKenzie2021AcousticAA,
  title={Acoustic Analysis and Dataset of Transitions Between Coupled Rooms},
  author={Thomas McKenzie and Sebastian J. Schlecht and Ville Pulkki},
  journal={ICASSP 2021 - 2021 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  year={2021},
  pages={481-485},
  note={{D}ata: \url{https://zenodo.org/record/4636068#.YhT-45PMJ6c}}
}

@article{McKenzie2021DatasetOS,
  title={Dataset of Spatial Room Impulse Responses in a Variable Acoustics Room for Six Degrees-of-Freedom Rendering and Analysis},
  author={Thomas McKenzie and Leo McCormack and Christoph Hold},
  journal={ArXiv},
  year={2021},
  volume={abs/2111.11882},
  note={{D}ata: \url{https://zenodo.org/record/5720724#.YhT_6JPMJ6c}}
}

@article{Eaton2016EstimationOR,
  title={Estimation of Room Acoustic Parameters: The ACE Challenge},
  author={James Eaton and Nikolay D. Gaubitch and Alastair H. Moore and Patrick A. Naylor},
  journal={IEEE/ACM Transactions on Audio, Speech, and Language Processing},
  year={2016},
  volume={24},
  pages={1681-1693},
  note={{D}ata: https://doi.org/10.5281/zenodo.6257551}
}

@article{di2021dechorate,
  title={dEchorate: a Calibrated Room Impulse Response Database for Echo-aware Signal Processing},
  author={Di Carlo, Diego and Tandeitnik, Pinchas and Foy, C{\'e}dric and Deleforge, Antoine and Bertin, Nancy and Gannot, Sharon},
  journal={arXiv preprint arXiv:2104.13168},
  year={2021},
  note={\url{https://doi.org/10.5281/zenodo.4626589}}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@INPROCEEDINGS{2017lippi,
  author={Lippi, Marco and Mamei, Marco and Mariani, Stefano and Zambonelli, Franco},
  booktitle={2017 IEEE 37th International Conference on Distributed Computing Systems (ICDCS)}, 
  title={Coordinating Distributed Speaking Objects}, 
  year={2017},
  volume={},
  number={},
  pages={1949-1960},
  doi={10.1109/ICDCS.2017.282}}
  
  @INPROCEEDINGS{2015mroueh,  author={Mroueh, Youssef and Marcheret, Etienne and Goel, 
  Vaibhava},  
  booktitle={2015 IEEE International Conference on Acoustics, 
  Speech and Signal Processing (ICASSP)},   
  title={Deep multimodal learning for Audio-Visual Speech Recognition},   
  year={2015},  volume={},  number={},  pages={2130-2134},  doi={10.1109/ICASSP.2015.7178347}}
  
  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%	
@inproceedings{dongtao_overview,
author = {Dong, Tao and Churchill, Elizabeth F. and Nichols, Jeffrey},
title = {Understanding the Challenges of Designing and Developing Multi-Device Experiences},
year = {2016},
isbn = {9781450340311},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/2901790.2901851},
doi = {10.1145/2901790.2901851},
abstract = {As the number of computing devices available to users continues to grow, personal computing increasingly involves using multiple devices together. However, support for multi-device interactions has fallen behind users' desire to leverage the diverse capabilities of the devices that surround them. In this paper, we report on an interview study of 29 designers and developers in which we investigate the barriers to creating useful, usable, and delightful multi-device experiences. We uncovered three key challenges: 1) the difficulty in designing the interactions between devices, 2) the complexity of adapting interfaces to different platform UI standards, and 3) the lack of tools and methods for testing multi-device user experiences. We discuss the technological and business factors behind these challenges and potential ways to lower the barriers they impose.},
booktitle = {Proceedings of the 2016 ACM Conference on Designing Interactive Systems},
pages = {62–72},
numpages = {11},
keywords = {developer experience, multichanneled services, design issues, multi-device experiences, crossmedia services, interviews, cross-device interactions},
location = {Brisbane, QLD, Australia},
series = {DIS '16}
}

@inproceedings{lienhart2003importance,
  title={On the importance of exact synchronization for distributed audio signal processing},
  author={Lienhart, Rainer and Kozintsev, Igor and Wehr, Stefan and Yeung, Minerva},
  booktitle={2003 IEEE International Conference on Acoustics, Speech, and Signal Processing, 2003. Proceedings.(ICASSP'03).},
  volume={4},
  pages={IV--840},
  year={2003},
  organization={IEEE}
}
  
% Change to ICASSP
@inproceedings{barber2021endtoend,
      title={End-to-end Alexa Device Arbitration}, 
      author={Jarred Barber and Yifeng Fan and Tao Zhang},
      year={2022},
      booktitle={2022 IEEE International Conference on Acoustics, Speech, and Signal Processing, 2022. Proceedings.(ICASSP 2022).},
      organization={IEEE}
}

@article{pasha2020distributed,
  title={Distributed microphone arrays, emerging speech and audio signal processing platforms: A review},
  author={Pasha, Shahab and Lundgren, Jan and Ritz, Christian and Zou, Yuexian},
  journal={Advances in Science, Technology and Engineering Systems},
  volume={5},
  number={4},
  pages={331--343},
  year={2020}
}

@inproceedings{michaud20203d,
  title={3D localization of a sound source using mobile microphone arrays referenced by SLAM},
  author={Michaud, Simon and Faucher, Samuel and Grondin, Fran{\c{c}}ois and Lauzon, Jean-Samuel and Labb{\'e}, Mathieu and L{\'e}tourneau, Dominic and Ferland, Fran{\c{c}}ois and Michaud, Fran{\c{c}}ois},
  booktitle={2020 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={10402--10407},
  year={2020},
  organization={IEEE}
}

@Article{locreview,
AUTHOR = {Liaquat, Muhammad Usman and Munawar, Hafiz Suliman and Rahman, Amna and Qadir, Zakria and Kouzani, Abbas Z. and Mahmud, M. A. Parvez},
TITLE = {Localization of Sound Sources: A Systematic Review},
JOURNAL = {Energies},
VOLUME = {14},
YEAR = {2021},
NUMBER = {13},
ARTICLE-NUMBER = {3910},
URL = {https://www.mdpi.com/1996-1073/14/13/3910},
ISSN = {1996-1073},
ABSTRACT = {Sound localization is a vast field of research and advancement which is used in many useful applications to facilitate communication, radars, medical aid, and speech enhancement to but name a few. Many different methods are presented in recent times in this field to gain benefits. Various types of microphone arrays serve the purpose of sensing the incoming sound. This paper presents an overview of the importance of using sound localization in different applications along with the use and limitations of ad-hoc microphones over other microphones. In order to overcome these limitations certain approaches are also presented. Detailed explanation of some of the existing methods that are used for sound localization using microphone arrays in the recent literature is given. Existing methods are studied in a comparative fashion along with the factors that influence the choice of one method over the others. This review is done in order to form a basis for choosing the best fit method for our use.},
DOI = {10.3390/en14133910}
}



